GRUtopia: Dream General Robots in a City at Scale

Recent works have been exploring the scaling laws in the field of Embodied AI. Given the prohibitive costs of collecting real-world data, we believe the Simulation-to-Real (Sim2Real) paradigm is a crucial step for scaling the learning of embodied models. This paper introduces project GRUtopia, the first simulated interactive 3D society designed for various robots. It features several advancements: (a) The scene dataset, GRScenes, includes 100k interactive, finely annotated scenes, which can be freely combined into city-scale environments. In contrast to previous works mainly focusing on home, GRScenes covers 89 diverse scene categories, bridging the gap of service-oriented environments where general robots would be initially deployed. (b) GRResidents, a Large Language Model (LLM) driven Non-Player Character (NPC) system that is responsible for social interaction, task generation, and task assignment, thus simulating social scenarios for embodied AI applications. (c) The benchmark, GRBench, supports various robots but focuses on legged robots as primary agents and poses moderately challenging tasks involving Object Loco-Navigation, Social Loco-Navigation, and Loco-Manipulation. We hope that this work can alleviate the scarcity of high-quality data in this field and provide a more comprehensive assessment of Embodied AI research. The project is available at https://github.com/OpenRobotLab/GRUtopia.

==> arxiv/supp_sections/APIs.tex <==

\section{Learning-based Control APIs}



We conduct extensive evaluations of the locomotion controllers\footnote{The locomotion policies of quadruped robots and humanoid robots are trained using Isaac Gym. As the training procedures are related to other works currently under review, we will not expose the learning details here due to confidentiality policies. The implementations will be released in the future for the benefit of the community.} on both the Unitree H1 and Aliengo Z1 robots. These tests are carried out in two distinct environments: an open flat terrain and a cluttered, furniture-rich setting. In the locomotion controller tests, the robot is required to follow a collision-free trajectory. As shown in Tab.~\ref{tab:APIs}, the robot is tasked with adhering to predefined paths on flat terrain. Results indicate a perfect success rate and low following error in these controlled conditions. However, when transitioning to real-world applications, even with collision-free ground truth paths, there is a significant drop in performance. The manipulation tasks also revealed significant performance degradation when moving from controlled tests to more practical scenarios. This disparity underscores the challenges of transferring controlled environment successes to real-world scenarios.

Our findings indicate a crucial gap between the performance of current RL-trained locomotion controllers in controlled environments versus real-world scenarios. This gap is evident in both locomotion and manipulation tasks. Consequently, we advocate for a more integrated research approach, combining low-level control studies with high-level task execution in realistic settings.



==> arxiv/supp_sections/clarifications.tex <==
\section*{Clarifications}
We would like to clarify a few mistakes in the main paper. In Fig.~\red{3}, ``World Information Manager'' should be ``World Knowledge Manager'' as introduced in lines 154-164. The metrics ``EC'' and ``SC'' in Tab.~\red{2-4} should be ``ECR'' and ``SCR'' as defined in lines 252-257. We will update the numbers reported in Tab.~\red{2-4} accordingly in the revision.


==> arxiv/supp_tables/ablation_dialogue_round.tex <==
\begin{wraptable}[10]{r}{7cm}
\centering
\renewcommand\arraystretch{1.1}
\vspace{-2.5ex}
\caption{\small
% 
The impact of allowed dialogue rounds on agent performance.
% 
} % \caption
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}|c|ccccc|@{}}
\hline
\multicolumn{1}{|c|}{\multirow{2}*{Round}} & \multicolumn{5}{c|}{Social Loco-Navigation}  \\
\cline{2-6}
~ & PL & SR & SPL & EC & RT \\
\hline
0 & 16.26 & 14.00 & 8.64 & - & 2.48\\
1 & 17.50 & 24.00 & 11.71 & 0.7 & 2.80\\
2 & 17.85 & 14.00 & 8.75 & 0.3 & 3.04\\
3 & 18.61 & 18.00 & 11.06 & 0.26 & 2.60\\
4 & 17.51 & 14.00 & 9.52 & 6.67 & 2.38\\
\hline
\end{tabular}
} % \resizebox
\label{tab:dialogue}
\end{wraptable}

==> arxiv/supp_tables/ablation_oracle.tex <==
\begin{table}
\centering
\renewcommand\arraystretch{1.1}
\caption{\small
% 
Impact of oracle actions on agent's performance.
% 
} % \caption
\vspace{0.5ex}
\resizebox{0.8\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}|c|c|cccc|ccccc|@{}}
\hline
\multirow{2}*{\#} & \multicolumn{1}{c|}{\multirow{2}*{Controller}} & \multicolumn{4}{c|}{Object Loco-Navigation} & \multicolumn{5}{c|}{Social Loco-Navigation}    \\
\cline{3-11}
~ & ~ & PL & SR & SPL & RT & PL & SR & SPL & ECR & RT \\
\hline
1 & RL-based & 23.82 & 8.00 & 4.26 & 0.89  \\
2 & Oracle &  \\
\hline
\end{tabular}
} % \resizebox
\vspace{-3ex}
\label{tab:oracle}
\end{table}

==> arxiv/supp_tables/more_baselines.tex <==
\begin{table}
\centering
\renewcommand\arraystretch{1.3}
\caption{\small
% 
Experimental results of more baselines on Object Loco-Navigation and Social Loco-Navigation. (PL: Path Length, \textbf{SR}: Success Rate, SPL: Success rate weighted by normalized inverse Path Length, ECR: Excluded Candidate Rate, RT: Reset Times)
% 
} % \caption
\vspace{1ex}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}|cc|cccc|cccc|ccccc|ccccc|@{}}
\hline
\multicolumn{2}{|c|}{\multirow{3}*{Method}} & \multicolumn{8}{c|}{Object Loco-Navigation} & \multicolumn{10}{c|}{Social Loco-Navigation}   \\
\cline{3-20}
~ & ~ & \multicolumn{4}{c|}{\texttt{validation}} & \multicolumn{4}{c|}{\texttt{test}} & \multicolumn{5}{c|}{\texttt{validation}} & \multicolumn{5}{c|}{\texttt{test}} \\
~ & ~ & PL & SR & SPL & RT & PL & SR & SPL & RT & PL & SR & SPL & ECR & RT & PL & SR & SPL & ECR & RT  \\
\hline

\multirow{2}*{\rotatebox{90}{VLM }} &\multicolumn{1}{|c|}{\multirow{2}*{InternVL-chat-1.5~\cite{chen2024far}}} & \multirow{2}*{12.77} & \multirow{2}*{8} & \multirow{2}*{5.45} & \multirow{2}*{0.67} & \multirow{2}*{10.85} & \multirow{2}*{5.5} & \multirow{2}*{3.88} & \multirow{2}*{0.23} & \multirow{2}*{15.19} & \multirow{2}*{0} &\multirow{2}*{ 0} & \multirow{2}*{0} & \multirow{2}*{6.67} & \multirow{2}*{16.80} & \multirow{2}*{0} & \multirow{2}*{0} & \multirow{2}*{0} & \multirow{2}*{6.35} \\
&\multicolumn{1}{|c|}{~}&&&&\multicolumn{1}{c|}{~}&&&&\multicolumn{1}{c|}{~}&&&&&\multicolumn{1}{c|}{~}&&&&&\multicolumn{1}{c|}{~}\\
\hline
\multirow{3}*{\rotatebox{90}{LLM }}&\multicolumn{1}{|c|}{Llama-3 8B~\cite{llama3}} & 25.97 & 10 & 7.21 & 0.84 & 23.32 & 15.5 & 10.96 & 0.57 & 20.77 & 5 & 3.49 & 17.69 & 1.54 & 21.42 & 11 & 6.26 & 7.21 & 1.89\\
~ &\multicolumn{1}{|c|}{InternLM-2-Chat~\cite{cai2024internlm2}} & 22.29 & 18 & 10.97 & 0.42 & 22.62 & 21.5 & 12.45 & 0.62 & 22.25 & 11 & 6.37 & 4.93 & 1.79 & 20.97 & 7.50 & 4.40 & 6.32 & 2.22\\
~ &\multicolumn{1}{|c|}{ChatGLM3~\cite{zeng2022glm}} & 22.75 & 22 & 12.97 & 0.60 & 23.78 & 22 & 11.68 & 0.74 & 21.13 & 8 & 4.61 & 7.1 & 2.06 & 20.36 & 11 & 6.97 & 0.13 & 2.25\\
\hline
\end{tabular}
} % \resizebox
\vspace{-3ex}
\label{tab:benchmark}
\end{table}

==> arxiv/supp_tables/scene_categories.tex <==

\begin{longtable}{| m{4cm} | m{5cm} |}
\caption{Details of scene categories in GRScenes.}\label{tab:scene_categories} \\
\hline
\textbf{Main Category} & \textbf{Sub-category} \\ 
\hline
Office Space & Office \\
 & Lobby \\
 & Pantry \\
 & Reception Room \\
 & Lecture Hall \\
\hline
Dining Space & Private Room \\
 & Cafe \\
 & Cafeteria \\
 & Milk Tea Shop \\
 & Hot Pot Restaurant \\
 & Chinese Restaurant \\
 & Teahouse \\
 & Buffet Restaurant \\
 & Western Restaurant \\
 & Dessert Bakery \\
 & Open Kitchen \\
 & Back Kitchen \\
 & Barbecue Restaurant \\
 & Fast Food Restaurant \\
 & Noodle Shop \\
 & Tavern \\
\hline
Entertainment Space & E-sports Room \\
 & Bar \\
 & Chess Room \\
 & KTV \\
 & Beauty Salon \\
 & Billiard Room \\
 & Nail Salon \\
 & Children's Playground \\
 & Cinema \\
 & Foot Bath Shop \\
 & Hair Salon \\
 & Script Murder \\
 & Internet Cafe \\
\hline
Commercial Space & Clothing Store \\
 & Sales Office \\
 & Live Broadcast Room \\
 & Supermarket \\
 & Mall \\
 & Bookstore \\
 & Convenience Store \\
 & Jewelry Store \\
 & Tobacco and Alcohol Store \\
 & Flower Shop \\
 & Tea Shop \\
 & Outdoor Stall \\
 & Pet Shop \\
 & Glasses Shop \\
 & Fruit Shop \\
 & Vegetable Market \\
 & Snack Shop \\
 & Pharmacy \\
 & Market \\
 & Maternal and Infant Store \\
 & Wedding Photography \\
 & Digital Store \\
 & Toy and Gift Store \\
 & Furniture Store \\
 & Exhibition Hall \\
\hline
Public Space & Public Toilet \\
 & Library \\
 & Museum \\
 & Command Center \\
 & Dressing Room \\
 & Locker Room \\
 & Bank \\
 & Activity Room \\
 & Workshop \\
 & Service Center \\
 & Honor Room \\
 & Gas Station \\
 & Airport \\
 & Station \\
 & Indoor Parking Lot \\
 & Government Offices \\
 & Religious Culture \\
 & Hospital \\
\hline
Hotel Space & Hotel \\
 & Homestay \\
\hline
Educational Space & School \\
 & Kindergarten \\
 & Classroom \\
 & Laboratory \\
 & Reading Room \\
\hline
General Space & Staircase \\
 & Elevator \\
 & Lobby \\
 & Corridor \\
 & Rest Area \\
 & Dormitory \\
 & Party Building Room \\
 & Atrium \\
\hline
Sports Space & Gym \\
 & Swimming Pool \\
 & Stadium \\
 & Yoga Room \\
\hline

\end{longtable}


==> arxiv/tables/ablation_dialogue_round.tex <==
\begin{wraptable}[8]{r}{5cm}
\centering
\renewcommand\arraystretch{1.1}
\vspace{-2.5ex}
\caption{\small
% 
The impact of allowed dialogue rounds on agent performance.
% 
} % \caption
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}|c|ccccc|@{}}
\hline
\multicolumn{1}{|c|}{\multirow{2}*{Round}} & \multicolumn{5}{c|}{Social Loco-Navigation}  \\
\cline{2-6}
~ & PL & SR & SPL & EC & RT \\
\hline
0 & 17.86 & 6.00 & 14.58 & - & 0.60 \\
1 & 21.90 & 10.00 & 6.06 & 0.79 & 1.20 \\
2 & 23.28 & 8.00 & 5.30 & 0.34 & 1.90 \\
3 & 20.48 & 17.00 & 13.28 & 0.50 & 1.40 \\
4 & 23.55 & 24.00 & 15.99 & 0.55 & 1.40 \\
\hline
\end{tabular}
} % \resizebox
\label{tab:dialogue}
\end{wraptable}
